Condorcet-Consistent and Approximately Strategyproof Tournament Rules

We consider the manipulability of tournament rules for round-robin tournaments of $n$ competitors. Specifically, $n$ competitors are competing for a prize, and a tournament rule $r$ maps the result of all $\binom{n}{2}$ pairwise matches (called a tournament, $T$) to a distribution over winners. Rule $r$ is Condorcet-consistent if whenever $i$ wins all $n-1$ of her matches, $r$ selects $i$ with probability $1$. We consider strategic manipulation of tournaments where player $j$ might throw their match to player $i$ in order to increase the likelihood that one of them wins the tournament. Regardless of the reason why $j$ chooses to do this, the potential for manipulation exists as long as $\Pr[r(T) = i]$ increases by more than $\Pr[r(T) = j]$ decreases. Unfortunately, it is known that every Condorcet-consistent rule is manipulable (Altman and Kleinberg). In this work, we address the question of how manipulable Condorcet-consistent rules must necessarily be - by trying to minimize the difference between the increase in $\Pr[r(T) = i]$ and decrease in $\Pr[r(T) = j]$ for any potential manipulating pair. We show that every Condorcet-consistent rule is in fact $1/3$-manipulable, and that selecting a winner according to a random single elimination bracket is not $\alpha$-manipulable for any $\alpha > 1/3$. We also show that many previously studied tournament formats are all $1/2$-manipulable, and the popular class of Copeland rules (any rule that selects a player with the most wins) are all in fact $1$-manipulable, the worst possible. Finally, we consider extensions to match-fixing among sets of more than two players.

==> conclusion.tex <==
\section{Conclusion}

In this paper we resolve the question of finding the optimal profitability of a bribe $\alpha$ that a 2-player coalition could obtain in tournaments. We exhibit tournaments that achieve lower bounds of $1/3$ and show that for the randomized single bracket elimination rule this is optimal. We also show a lower bound for the case of $k$-player coalitions, but fail to come up with a rule that matches this. 

\begin{conjecture}
There exists a rule $r$ that is $k-$SNM-$\frac{k-1}{2k-1}$. 
\end{conjecture}

We believe this conjecture to be hard to resolve and pose the following related open question instead. 

\vbox{%
\noindent
\begin{quote}
\begin{description}
\item Does there exist a rule $r$ such that for every $k$, it is $k$-SNM-$\frac{1}{2}$?
\end{description}
\end{quote}
}

In other words, is there a rule such that has a provable, constant profitability value $\alpha$  that is independent of the coalition size? 
